Group-Harmonic and Group-Closeness Maximization -- Approximation and Engineering

Centrality measures characterize important nodes in networks. Efficiently computing such nodes has received a lot of attention. When considering the generalization of computing central groups of nodes, challenging optimization problems occur. In this work, we study two such problems, group-harmonic maximization and group-closeness maximization both from a theoretical and from an algorithm engineering perspective. On the theoretical side, we obtain the following results. For group-harmonic maximization, unless $P=NP$, there is no polynomial-time algorithm that achieves an approximation factor better than $1-1/e$ (directed) and $1-1/(4e)$ (undirected), even for unweighted graphs. On the positive side, we show that a greedy algorithm achieves an approximation factor of $\lambda(1-2/e)$ (directed) and $\lambda(1-1/e)/2$ (undirected), where $\lambda$ is the ratio of minimal and maximal edge weights. For group-closeness maximization, the undirected case is $NP$-hard to be approximated to within a factor better than $1-1/(e+1)$ and a constant approximation factor is achieved by a local-search algorithm. For the directed case, however, we show that, for any $\epsilon<1/2$, the problem is $NP$-hard to be approximated within a factor of $4|V|^{-\epsilon}$. From the algorithm engineering perspective, we provide efficient implementations of the above greedy and local search algorithms. In our experimental study we show that, on small instances where an optimum solution can be computed in reasonable time, the quality of both the greedy and the local search algorithms come very close to the optimum. On larger instances, our local search algorithms yield results with superior quality compared to existing greedy and local search solutions, at the cost of additional running time. We thus advocate local search for scenarios where solution quality is of highest concern.

==> dump.tex <==
% Drop multi-swaps, might be mentioned as future work
\subsection{Multi-swaps}
In the multi-swap strategy, up to $1 < p < k$ vertices can be swapped simultaneously
at each iteration. Algorithm~\ref{algo:local-search-multiswap} shows an analogous
approach as in the single-swap case. We first remove $p$ vertices from $S$ so that
the farness increment is minimum (lines~\ref{line:p-removals} to~\ref{line:p-removals-end}).
Afterwards, we add $p$ vertices to $S$ that minimize $\GF(S)$. If the decrement of $\GF(S)$
\wrt the previous iteration is less than a factor of $\epsilon/Q$, the algorithm terminates.
Now $Q\le\binom{n - k + p}{p}$, as Algorithm~\ref{algo:local-search-multiswap} does not consider
all the neighboring solutions.

\paragraph{Comments}
The multi-swap algorithm described here is not exactly equivalent to the multi-swap algorithm for $k$-median.
In particular:
\begin{itemize}
    \item we do not consider all neighboring solutions as in the single swap case, at each iterations
        we test at most $n-k$ of them.
    \item it is not yet clear if the local optimum returned by Algorithm~\ref{algo:local-search-multiswap} has the same
        locality gap as the algorithm described in~\cite{AryaGKMMP04} and, if so, how to prove it
\end{itemize}

\begin{algorithm}
\caption{Overview of the multi-swap algorithm}
% \textbf{Input:} $G=(V, E)$ connected and undirected, arbitrary $S\subset V$, $\epsilon > 0$, integer $0<p<|S|$.}
\label{algo:local-search-multiswap}
\begin{algorithmic}[1]
\State $k \gets |S|$
\Repeat\label{line:outer-repeat-multiswap}
    \State $S_\mathrm{old} \gets S$
    \State $\GF(S_\mathrm{old}) \gets SSSP(S_\mathrm{old})$
    \For{$i \gets 1$ \textbf{to} $p$}\Comment{Remove $p$ vertices from $S$ so that $\GF(S_\mathrm{old}) - \GF(S)$ is minimized.}\label{line:p-removals}
    \State $u \gets \argmin_{u\in S}\GF(S_{-u}) - \GF(S)$
    \State $S \gets S_{-u}$\label{line:p-removals-end}
    \EndFor
    \State $\GF(S) \gets SSSP(S)$
    \State approximate $|D_v|$ for all $V \setminus S$
    \State $PQ \gets$ max-PQ with key $|D_v|$ and value $v$
    \State continue $\gets$ \false
    \Repeat
    \State $v \gets PQ.\texttt{extract\_max()}$
    \State $S \gets S^{+v}$
    \State $\GF(S)\gets$ pruned SSSP from $v$\Comment{Compute exact farness decrement.}
    \If{$|S| = k$}
        \If{$\GF(S) \le (1 - \frac{\epsilon}{Q})\cdot\GF(S_\mathrm{old})$}
            \State continue $\gets$ \texttt{true}
            \State\textbf{break}
        \Else
            \State $u \gets \argmin_{u\in S}\GF(S_{-u}) - \GF(S)$
            \State $S \gets S_{-u}$
            \State update $\GF(S)$
        \EndIf
    \EndIf
    \Until{$PQ$ is empty}
\Until{\texttt{not} continue}
\State\Return$S$
\end{algorithmic}
\end{algorithm}

Idea: to get a good initial solution, run the BigData'19 algorithm with a high-quality setting.
Then run the approximation algorithm to improve the set. Hopefully, almost no swaps
will be necessary.

\paragraph{Comments and possible improvements}
\begin{itemize}
    \item In the last iteration of the algorithm, the loop at
        line~\ref{line:inner-repeat} will iterate over all the vertices in
        $V\setminus S$. If we had a lower bound for $\GF(S) - \GF(S^{+v})$
        instead of an approximation of $|D_v|$, we could stop earlier and save
        time.
    \item $k$-means++ could give a better initialization for $S$ (i.e., might reduce
        the number of swaps required to converge to a local optimum), but it is
        unclear if this would bring a real improvement of running time or
        quality. Time permitting, we should try it.
\end{itemize}


